On conformal maps from multiply connected domains onto lemniscatic domains

We study conformal maps from multiply connected domains in the extended complex plane onto lemniscatic domains. Walsh proved the existence of such maps in 1956 and thus obtained a direct generalization of the Riemann mapping theorem to multiply connected domains. For polynomial pre-images of simply connected sets we derive a construction principle for Walsh's conformal map in terms of the Riemann map for the simply connected set. Moreover, we explicitly construct examples of Walsh's conformal map for certain radial slit domains and circular domains.

==> sect_map_disks.tex <==
%% Section -- Lemniscatic map for two equal disks

\section{Lemniscatic map for two equal disks}
\label{sect:map_disks}

In this section we analytically construct the lemniscatic map of a set $E$ that 
is the union of two disjoint equal disks.
Let us denote by $D_r(z_0) = \{ z \in \C : \abs{z-z_0} \leq r \}$ the closed 
disk with radius $r > 0$ and center $z_0 \in \C$.
By Lemma~\ref{lem:linear_trafo} we can assume without loss of generality that 
$E = D_r(z_0) \cup D_r(-z_0)$ with real $z_0$ and $0 < r < z_0$.
Let $P(z) = \alpha z^2 + \alpha_0$ with $\alpha > 0$, then
\begin{equation*}
\Omega = \{ \alpha (z_0 + \rho e^{it})^2 + \alpha_0 : 0 \leq \rho \leq r,
0 \leq t \leq 2 \pi \}
\end{equation*}
is a simply connected compact set with $E = P^{-1}(\Omega)$,
so that in principle we could apply Theorem~\ref{thm:pre-images}. 
However, the Riemann map for the set $\Omega$ seems not to be readily 
available.  Therefore, we directly construct the lemniscatic map as a 
composition of certain conformal maps.  The main ingredients are the map from 
the exterior of two disks onto the exterior of two intervals and from there 
onto a lemniscatic domain (according to Corollary~\ref{cor:radial_slits}).

We need the following conformal map from~\cite[pp.~293--295]{Nehari1952}.

\begin{lemma} \label{lem:annulus_to_slit_plane}
Let $0 < \rho < 1$ and define
\begin{equation}
L = L(\rho) \coloneq 2 \rho \prod_{n=1}^\infty \Big( \frac{1 + \rho^{8n}}{1 +
\rho^{8n-4}} \Big)^2, \label{eqn:formula_L}
\end{equation}
and the complete elliptic integral of the first kind
\begin{equation}
K = K(k) \coloneq \int_0^1 \frac{dt}{ \sqrt{(1 - t^2) (1 - k^2 t^2)} } \quad 
\text{with } k \coloneq L^2.
\label{eqn:K}
\end{equation}
Then the function
\begin{equation}
w = f(z) = L \sn \Big(\frac{2K}{\pi} i \log \Big(\frac{z}{\rho}\Big) + K; k\Big)
\label{eqn:annu_to_slit_disc}
\end{equation}
is a bijective and conformal map from the annulus $\rho < \abs{z} < \rho^{-1}$ 
onto the $w$-plane with the slits $-\infty < w \leq -\tfrac{1}{L}$, $-L \leq w 
\leq L$ and $\tfrac{1}{L} \leq w < \infty$.
Further, we have $f(-1) = -1$ and $f'(-1) = (1-L^2) \tfrac{2K}{\pi} > 0$, and
$f(z^{-1}) = (f(z))^{-1}$.
\end{lemma}

\begin{proof}
See~\cite[pp.~293--295]{Nehari1952} for the existence and mapping properties of
$f$.  Note that $f$ is independent of the choice of the branch of the 
logarithm.  By construction $f$ is also symmetric with respect to the real axis 
and to the unit circle, i.e., $f(z) = \overline{ f(\overline{z}) }$, and
$f(z) = 1 / \overline{ f( 1/\overline{z} ) }$.
This implies $f(1/z) = 1 / \overline{ f(\overline{z}) } = 1/f(z)$.

It remains to compute $f(-1)$ and $f'(-1)$.  Recall the identity
\begin{equation*}
\sn'(z; k) = \cn(z; k) \dn(z; k),
\end{equation*}
where $\cn(z; k) = \sqrt{1 - \sn(z; k)^2}$, 
$\cn(0) = 1$, 
and $\dn(z) = \sqrt{1 - k^2 \sn(z; k)^2}$, $\dn(0) = 1$.  We compute
\begin{equation*}
f'(z) = L \cn(\zeta(z); k) \dn(\zeta(z); k) \frac{2K}{\pi} i \frac{1}{z}, \quad 
\text{where} \quad
\zeta(z) = \frac{2 K}{\pi} i \log \Big( - i \frac{z}{\rho} \Big).
\end{equation*}
For $z = -1$ we have $\zeta(-1) = -K - i \frac{2K}{\pi} \log(\rho) \eqcolon -K 
+ i \frac{K'}{2}$; see~\cite[p.~294]{Nehari1952}.  With the special values
\begin{equation*}
\sn(K + i \tfrac{K'}{2}; k) = \frac{1}{\sqrt{k}}, \quad
\cn(K + i \tfrac{K'}{2}; k) = -i \sqrt{\frac{1}{k}-1}, \quad
\dn(K + i \tfrac{K'}{2}; k) = \sqrt{1-k},
\end{equation*}
see \cite[p.~381]{MagnusOberhettingerSoni1966} or \cite[p.~145]{Tricomi1948},
and the identities
\begin{equation*}
\sn(z+2K; k) = - \sn(z; k), \quad
\cn(z+2K; k) = - \cn(z; k), \quad
\dn(z+2K; k) = \dn(z; k),
\end{equation*}
see \cite[p.~500]{WhittakerWatson1962}, we obtain
\begin{equation*}
\begin{split}
f(-1) &= L \sn \Big( - K + i \frac{K'}{2}; k \Big) = - L \frac{1}{\sqrt{k}}
= -1, \\
f'(-1) &= L i \sqrt{\frac{1-k}{k}} \sqrt{1-k} \frac{2K}{\pi} i (-1)
= L \frac{1-k}{\sqrt{k}} \frac{2K}{\pi} = (1-L^2) \frac{2K}{\pi} > 0.
\end{split}
\end{equation*}
In the last equalities we used $k = L^2$.
\eop
\end{proof}



We now construct the lemniscatic map of the exterior of two disjoint equal 
disks.

\begin{theorem} \label{thm:ext_map_2_disks}
Let $r, z_0 \in \R$ with $0 < r < z_0$, and $E = D_r(z_0) \cup D_r(-z_0)$.
Let $T$ be the M\"{o}bius transformation
\begin{equation*}
T(z) = \frac{\alpha+z}{\alpha-z}, \quad \alpha = \sqrt{z_0^2 - r^2} > 0, 
% \label{eqn:Moebius_alpha}
\end{equation*}
$f$, $K$, $L$ be given as in Lemma~\ref{lem:annulus_to_slit_plane} with
\begin{equation*}
0 < \rho = \frac{\sqrt{z_0+r} - \sqrt{z_0-r}}{\sqrt{z_0+r} + \sqrt{z_0-r}} < 1,
\end{equation*}
and let $\Phi_1$ be the lemniscatic map from~\eqref{eqn:Phi_radial_slits} for
$n = 2$, with
\begin{equation}
C = \frac{2 K \alpha}{\pi} (1-L)^2, \quad
D = \frac{2 K \alpha}{\pi} (1+L)^2.
\label{eqn:CD_twodisks}
\end{equation}

Then
\begin{equation}
\Phi(z) = \Phi_1 ( f'(-1) \cdot (T^{-1} \circ f \circ T)(z) )
\label{eqn:Phi_disks}
\end{equation}
is the lemniscatic map of $E$ with corresponding lemniscatic domain
\begin{equation}
\cL = \left\{ w \in \widehat{\C} :
\Big\lvert w^2 - \Big( \frac{2K\alpha}{\pi} (1+L^2) \Big)^2 
\Big\rvert^\frac{1}{2}
> \sqrt{2 L (1+L^2)} \frac{2 K \alpha}{\pi} \right\},
\label{eqn:cL_two_disks}
\end{equation}
and hence, in particular, $c(E) = \sqrt{2 L (1+L^2)} \frac{2 K \alpha}{\pi}$.
\end{theorem}

\begin{proof}
Our proof is constructive.  First, $\Phi$ is obtained as composition of 
conformal maps which map $\widehat{\C} \backslash E$ to a lemniscatic domain.  
In a second step, we show that $\Phi$ is normalized as 
in~\eqref{eqn:normalization_Phi}, and thus is a lemniscatic map.
The first steps in the construction, namely $T^{-1} \circ f \circ T$, modify 
and generalize a conformal map in~\cite[p.~297]{Nehari1952}, and are 
illustrated in Figure~\ref{fig:map_two_disks}.

\input{fig_map_two_disks}


Since $T$ maps the points $-\alpha, 0, \alpha$ to $0, 1, \infty$, respectively, 
$T$ maps $\R$ to $\R$ (with same orientation).
We compute the images of the two disks under $z_1 = T(z)$.
Let
\begin{equation*}
\rho \coloneq T(-z_0+r)
= \frac{ \sqrt{z_0+r} - \sqrt{z_0-r} }{\sqrt{z_0+r} + \sqrt{z_0-r}} \in\; ]0,1[.
\end{equation*}
A short computation shows that $T(-z_0-r) = -\rho$.
Since the circle $\abs{z+z_0} = r$ cuts the real line in a right angle, this 
holds true for its image under $T$, and $T$ maps the circle 
$\abs{z+z_0} = r$ onto the circle $\abs{z_1} = \rho$.
Further, $T(-z) = 1/T(z)$ implies that $T$ maps $\abs{z-z_0} = r$ to 
$\abs{z_1} = \frac{1}{\rho}$.  Hence we see that $T$ maps $\widehat{\C} 
\backslash E$ onto the annulus $\frac{1}{\rho} < \abs{z_1} < \rho$.

This annulus is mapped by $z_2 = f(z_1)$ onto the complex plane with the slits 
$-\infty \leq z_2 \leq -\tfrac{1}{L}$, $-L \leq z_2 \leq L$ and $\tfrac{1}{L} 
\leq z_2 \leq \infty$, where $L = L(\rho)$ is given by~\eqref{eqn:formula_L}; 
see Lemma~\ref{lem:annulus_to_slit_plane}.

For $T^{-1}(z_2) = \alpha \frac{z_2-1}{z_2+1}$ we have $T^{-1}(1/z_2) = - 
T^{-1}(z_2)$.  Then, setting for brevity $b = \tfrac{1-L}{1+L}$, we compute
\begin{equation*}
T^{-1}(L^{-1}) = \alpha b, \quad
T^{-1}(-L^{-1}) = \alpha b^{-1}, \quad
T^{-1}(-L) = - \alpha b^{-1}, \quad
T^{-1}(L) = - \alpha b.
\end{equation*}
This shows that $T^{-1}$ maps the $z_2$-plane with the slits $-\infty \leq z_2 
\leq -L^{-1}$, $-L \leq z_2 \leq L$ and $L^{-1} \leq z_2 \leq \infty$ onto the 
$z_3$-plane with the two slits $[- \alpha b^{-1}, -\alpha b]$ and 
$[\alpha b, \alpha b^{-1}]$.
Multiplying with $f'(-1)$ we obtain the exterior of $[-D, -C] \cup [C, D]$, 
with $C$ and $D$ as in~\eqref{eqn:CD_twodisks}.
The lemniscatic map for this set is $\Phi_1$ from~\eqref{eqn:Phi_radial_slits}
with lemniscatic domain $\cL$ given by~\eqref{eqn:cL_radial_slits}.
A short calculation shows that $\cL$ has the form~\eqref{eqn:cL_two_disks}.

This shows that $\Phi : \widehat{\C} \backslash E \to \cL$ is a bijective and 
conformal map onto a lemniscatic domain, and it remains to 
verify~\eqref{eqn:normalization_Phi}.

We have $\Phi(\infty) = \infty$, since $T(\infty) = -1$ and $f(-1) = -1$, see 
Lemma~\ref{lem:annulus_to_slit_plane}, and since $\Phi_1$ 
satisfies the normalization in~\eqref{eqn:normalization_Phi}.
Next we show that $\Phi'(\infty) = 1$.  Let us begin with the derivative of
$g = T^{-1} \circ f \circ T$ at $z \neq \infty$, which is
\begin{equation*}
g'(z) = (T^{-1})'(f(T(z))) \cdot f'(T(z)) \cdot T'(z).
\end{equation*}
We compute $T'(z) = \frac{2 \alpha}{(\alpha-z)^2}$ and $(T^{-1})'(z) =
\frac{2 \alpha}{(z+1)^2}$, so that
\begin{equation*}
\begin{split}
(T^{-1})'(f(T(z))) \cdot T'(z)
&= (f(T(z)) - f(-1))^{-2} \frac{4 \alpha^2}{(\alpha-z)^2} \\
&= \Big( \frac{f(T(z)) - f(-1)}{T(z)-(-1)} \Big)^{-2}
\frac{4 \alpha^2}{ (T(z)+1)^2 (\alpha-z)^2} \\
&= \Big( \frac{f(T(z)) - f(-1)}{T(z)-(-1)} \Big)^{-2}.
\end{split}
\end{equation*}
We therefore find
\begin{equation*}
g'(\infty) = \lim_{z \to \infty} g'(z) 
= \lim_{z \to \infty} f'(T(z)) \Big( \frac{f(T(z)) - f(-1)}{T(z)-(-1)} 
\Big)^{-2} = \frac{1}{f'(-1)}.
\end{equation*}
This implies $\Phi'(\infty) = \Phi_1'(\infty) f'(-1) g'(\infty) = 1$, so that
$\Phi(z) = z + \cO(1)$ near infinity.
We further show that $\Phi$ is odd, so that the constant term in the Laurent 
series at infinity vanishes, showing~\eqref{eqn:normalization_Phi}.
The function $f$ satisfies $f(1/z) = 1/f(z)$; see 
Lemma~\ref{lem:annulus_to_slit_plane}.  Together with $T(-z) = 
1/T(z)$ and $T^{-1}(1/w) = - T^{-1}(w)$ this gives
\begin{equation*}
g(-z) = T^{-1}( f( T(-z) ) ) = T^{-1}( f(1/T(z)) ) = T^{-1} ( 1/f(T(z)) )
= - g(z).
\end{equation*}
Since also $\Phi_1$ is odd, which can be seen either from 
Lemma~\ref{lem:E_symm} or directly from~\eqref{eqn:Phi_radial_slits}, 
$\Phi$ is an odd function and is normalized as
in~\eqref{eqn:normalization_Phi}.
\eop
\end{proof}

Note that the construction in the proof of Theorem~\ref{thm:ext_map_2_disks} 
can be generalized to doubly connected domains $\cK = \widehat{\C} \backslash 
E$ as follows.
Let $h : \cK \to \{ w \in \C : 1/\rho < \abs{w} < \rho \}$ be a bijective 
conformal map that satisfies $\abs{h(\infty)} = 1$.  In this case we can assume 
(after rotation) that $h(\infty) = -1$.  We then have
\begin{equation*}
h(z) = -1 + a_1 / z + \cO(1/z^2) \quad \text{for } z \text{ near infinity},
\end{equation*}
with $a_1 \neq 0$ since $h$ is conformal.
Let $S(z) = \frac{z-1}{z+1}$.  Then the lemniscatic map of $E$ is given by
\begin{equation*}
\Phi(z) = \Phi_1 \left( - \frac{a_1 f'(-1)}{2} (S \circ f \circ h)(z) \right) + 
\beta
\end{equation*}
with $f$ as in Lemma~\ref{lem:annulus_to_slit_plane}, $\Phi_1$ the lemniscatic 
map of two (possibly rotated) intervals of same length, and $\beta \in \C$ is 
chosen so that the normalization~\eqref{eqn:normalization_Phi} holds.





In Figure~\ref{fig:disks} we plot the sets $E = E(z_0, r)$ for $z_0 = 1$ and $r 
= 0.5$, $0.7$ and $0.9$ (left) and the corresponding lemniscatic domains 
(right).  We evaluated the complete elliptic integral of the first 
kind~\eqref{eqn:K} using the MATLAB function \verb|ellipk|.  The product in the 
formula~\eqref{eqn:formula_L} for $L$ converges very quickly, so that it 
suffices to compute the first few terms in order to obtain the correct value 
up to machine precision.

\begin{figure}
\centerline{
\includegraphics[width=0.5\textwidth]{figures/2disks}
\includegraphics[width=0.5\textwidth]{figures/2disks_lem}
}
\caption{Illustration of Theorem~\ref{thm:ext_map_2_disks}.}
\label{fig:disks}
\end{figure}



%% End of section
